An Application of Pseudo-Log-Likelihoods to Natural Language Scoring

Language models built using semi-supervised machine learning on large corpora of natural language have very quickly enveloped the fields of natural language generation and understanding. In this paper we apply a zero-shot approach independently developed by a number of researchers now gaining recognition as a significant alternative to fine-tuning for evaluation on common sense tasks. A language model with relatively few parameters and training steps compared to a more recent language model (T5) can outperform it on a recent large data set (TimeDial), while displaying robustness in its performance across a similar class of language tasks. Surprisingly, this result is achieved by using a hyperparameter-free zero-shot method with the smaller model, compared to fine-tuning to the larger model. We argue that robustness of the smaller model ought to be understood in terms of compositionality, in a sense that we draw from recent literature on a class of similar models. We identify a practical cost for our method and model: high GPU-time for natural language evaluation. The zero-shot measurement technique that produces remarkable stability, both for ALBERT and other BERT variants, is an application of pseudo-log-likelihoods to masked language models for the relative measurement of probability for substitution alternatives in forced choice language tasks such as the Winograd Schema Challenge, Winogrande, and others. One contribution of this paper is to bring together a number of similar, but independent strands of research. We produce some absolute state-of-the-art results for common sense reasoning in binary choice tasks, performing better than any published result in the literature, including fine-tuned efforts. We show a remarkable consistency of the model's performance under adversarial settings, which we argue is best explained by the model's compositionality of representations.

==> tasks.tex <==
\subsection{Tasks}
\begin{enumerate}
    \item Abductive NLI (aNLI)  \cite{bhagavatula2020abductive} is cast as a natural language inference (NLI) task, in which the beginning and the ending of a story are provided, and two possible hypotheses relating the beginning and ending, of which one is more plausible, are given as choices for the system. The dataset consists of nearly 170k entries.
\item CommonsenseQA (CSQA) \cite{talmor2019commonsenseqa} tests common sense knowledge under a broad range of categories. Each entry contains a question and 5 answer candidates. The questions are crowdsourced based on a subgraph from ConceptNet, and the answer candidates draw from ConceptNet notes with additional crowdsourced distractor words.

\item PhysicalIQA (PIQA) \cite{bisk2020piqa} is a binary choice
question answering dataset which targets physical reasoning. Given a question as input, the system must select the more plausible out of two possible continuations.
\item SocialIQA (SIQA) \cite{sap2019social} is also a question answering dataset which requires reasoning about social interactions. Each entry contains a context, a question, and 3
answer candidates. The context is derived from the ATOMIC knowledge graph \cite{sap2019atomic} and the questions are generated based on nine templates (corresponding to the relations in ATOMIC), with answers that are crowdsourced.
\item  WinoGrande (WG) \cite{sakaguchi2020winogrande} is a large-scale dataset of 44k binary pronoun resolution problems, inspired by the original WSC but adjusted to improve both the scale and the difficulty of the dataset. The key steps of dataset construction are (1) a carefully designed crowdsourcing
procedure, followed by (2) systematic bias reduction against a finetuned RoBERTa model by adversarial filtering.
\end{enumerate}
